NeuroVectorizer: End-to-End Vectorization with Deep Reinforcement Learning

One of the key challenges arising when compilers vectorize loops for today's SIMD-compatible architectures is to decide if vectorization or interleaving is beneficial. Then, the compiler has to determine how many instructions to pack together and how many loop iterations to interleave. Compilers are designed today to use fixed-cost models that are based on heuristics to make vectorization decisions on loops. However, these models are unable to capture the data dependency, the computation graph, or the organization of instructions. Alternatively, software engineers often hand-write the vectorization factors of every loop. This, however, places a huge burden on them, since it requires prior experience and significantly increases the development time. In this work, we explore a novel approach for handling loop vectorization and propose an end-to-end solution using deep reinforcement learning (RL). We conjecture that deep RL can capture different instructions, dependencies, and data structures to enable learning a sophisticated model that can better predict the actual performance cost and determine the optimal vectorization factors. We develop an end-to-end framework, from code to vectorization, that integrates deep RL in the LLVM compiler. Our proposed framework takes benchmark codes as input and extracts the loop codes. These loop codes are then fed to a loop embedding generator that learns an embedding for these loops. Finally, the learned embeddings are used as input to a Deep RL agent, which determines the vectorization factors for all the loops. We further extend our framework to support multiple supervised learning methods. We evaluate our approaches against the currently used LLVM vectorizer and loop polyhedral optimization techniques. Our experiments show 1.29X-4.73X performance speedup compared to baseline and only 3% worse than the brute-force search on a wide range of benchmarks.

==> background.tex <==
\section{Background}
\label{bg}
\subsection{Reinforcement Learning}% and PCA}
One of the promising machine learning approaches is reinforcement learning (RL), in which an agent learns by continually interacting with an environment~\cite{kaelbling1996reinforcement}. Using a neural network in conjunction with RL, is called deep RL. Deep models allow RL algorithms to solve complex problems in an end-to-end fashion, handle unstructured environments, learn complex functions, or predict actions in states that have not been visited in the past. Deep RL is gaining wide interest recently due to its success in robotics, Atari games, and superhuman capabilities~\cite{mnih2013playing,doya2000reinforcement,kober2013reinforcement,peters2003reinforcement,hajali2019deep}. Deep RL was the key technique behind defeating the human European champion in the game of Go, which has long been viewed as the most challenging of classic games for artificial intelligence~\cite{silver2016mastering}. 

In RL, the agent observes the state of the environment, and based on this state/observation takes an action. The ultimate goal is to compute a policy ($\pi^*$)--a mapping between the environment states and actions--that maximizes expected reward:
\begin{align}
\label{eq:MDP}
    \pi^* = \argmaxA_\pi \mathbb{E}_{\tau{\raise.05ex\hbox{$\scriptstyle\mathtt{\sim}$}}\pi(\tau)} \left[\tau \right].
\end{align}
where $\tau$ is a sequence of states and actions that define a single episode.

If the number of steps the RL agent has to take before the environment terminates is one, the problem is called Contextual Bandits. In Contextual Bandits the learner tries to find a single best action in the current state. It involves both learning to search for best actions and trial-and-error. 

One of the promising deep RL methods to derive a good, stable, and easy to use policy is proximal policy optimization (PPO)~\cite{schulman2017proximal}. PPO computes a gradient update at each step that minimizes the cost function while ensuring the deviation from the previous policy is relatively small.

%Principal component analysis (PCA) is a statistical procedure that uses an orthogonal transformation to convert a set of observations of possibly correlated variables into a set of values of linearly uncorrelated variables called principal components. PCA performs a linear mapping of the data to a lower-dimensional space in such a way that the variance of the data in the low-dimensional representation is maximized.
\subsection{Related Work}
Using machine learning for optimization in compilers is not new~\cite{ashouri2018survey,wang2018machine}. For example, in~\cite{haj2019autophase,fursin2011milepost} deep supervised and RL methods were proposed to overcome the phase ordering challenge. In~\cite{stock2012using} for example, multiple machine learning methods for automatic vectorization have been proposed. Our work is different in that it the first to propose deep RL to explore the vectorization space. Second, all these works still rely on hand extracted features from the program such as the arithmetic intensity, memory operations, number of different instruction and the distance between producer and consumer. These features however do not fully represent the original code. By contrast, our work addresses the automatic vectorization end to end from the text code itself to the optimal factors without any loss of information. 

Automatic vectorization with other methods was also proposed. For example, the currently implemented cost model in LLVM and recently proposed cost model in~\cite{tian2016llvm} rely on predefined cost functions that calculate the expected execution time of a vectorized loop based on a linear formula from the instruction distribution. Polly~\cite{grosser2012polly} uses an abstract mathematical representation based on integer polyhedra to analyze and optimize the memory access pattern of a program. Polly performs classical loop transformations, especially tiling and loop fusion to improve data-locality. These transformations also simplify vectorization decisions for the compiler.

% \subsection{Code2vec}
\subsection{Learning Code Embeddding}
There are multiple ways to generate/learn an embedding for input code. One example is to use Polly's mathematical representation of loops as an embedding. In this work we use code2vec~\cite{alon2019code2vec}. Code2vec is a neural network model for representing snippets of code as continuous distributed vectors. Code2vec represents a code snippet as a single fixed-length code vector, which can be used to
predict semantic properties of the snippet. These vectors capture many characteristics of the code, such as semantic similarities, combinations, and analogies. Code is first decomposed to a collection of paths in its abstract syntax tree. Then, the network simultaneously learns the atomic representation of each path while learning how to aggregate a set of them.

